Why We Feel: Breaking Boundaries in Emotional Reasoning with Multimodal Large Language Models

Most existing emotion analysis emphasizes which emotion arises (e.g., happy, sad, angry) but neglects the deeper why. We propose Emotion Interpretation (EI), focusing on causal factors-whether explicit (e.g., observable objects, interpersonal interactions) or implicit (e.g., cultural context, off-screen events)-that drive emotional responses. Unlike traditional emotion recognition, EI tasks require reasoning about triggers instead of mere labeling. To facilitate EI research, we present EIBench, a large-scale benchmark encompassing 1,615 basic EI samples and 50 complex EI samples featuring multifaceted emotions. Each instance demands rationale-based explanations rather than straightforward categorization. We further propose a Coarse-to-Fine Self-Ask (CFSA) annotation pipeline, which guides Vision-Language Models (VLLMs) through iterative question-answer rounds to yield high-quality labels at scale. Extensive evaluations on open-source and proprietary large language models under four experimental settings reveal consistent performance gaps-especially for more intricate scenarios-underscoring EI's potential to enrich empathetic, context-aware AI applications. Our benchmark and methods are publicly available at: https://github.com/Lum1104/EIBench, offering a foundation for advanced multimodal causal analysis and next-generation affective computing.

==> sections/method.tex <==
\section{Coarse-to-Fine Self-Ask Method}
% 介绍各个模块，包括问题解析、问题重建方式、general self-ask、scenario specific self-ask
% general self-ask目的是为了让模型获得对人物情感的粗略理解，因为主要问的是和周围人交互，以及面部表情、body language
% scenario specific self-ask则是针对特定场景提问（此处使用了GPT4 api结合LLaVA-34B模型生成问题）
In this section, we introduce the detailed methodology for our Coarse-to-Fine Self-Ask (CFSA) method (Appendix Figure~\ref{dataset_pipeline}), designed to address the Emotion Interpretation (EI) task. Our approach involves breaking down complex, implicit user questions into a series of simple VQA queries. CFSA comprises three main components: User Question Preprocessing (Sec.~\ref{sec:user_question_preprocess}), General Self-Ask Thinking (Sec.~\ref{sec:general_self_ask}), and Scenario-Specific Self-Ask Thinking (Sec.~\ref{sec:scenario_spe_self_ask}).

\subsection{User Question Preprocessing}
\label{sec:user_question_preprocess}

Given a user question $x_{query}$, the CFSA method parses the $x_{query}$ into two aspects: $p_{p}$, identifying the person inquired about by the user, and $p_r$, signifying the user's request. Subsequently, a caption $p_{cap}$ pertaining to $p_{p}$ is concatenated with $p_r$ for the question reconstruction $x_{rec}$:

\begin{equation}
x_{rec} = Concat(p_{cap}, p_{r})
\end{equation}

\subsection{General Self-Ask Thinking}
\label{sec:general_self_ask}
The purpose of ``General Self-Ask Thinking'' is to equip the model with a comprehensive understanding of the entire image. To achieve this, we employ GPT-4 to generate 10 questions to enhance its understanding of the image. Instead of directly inputting the image into the model, we present a caption to provide a high-level overview of the scene. This approach prevents the model from being overwhelmed by visual information and encourages the formulation of more general questions. Following the analysis of the answers, we have identified four common themes for the general self-ask question $x_{gen}$:
\begin{itemize}
\item \textbf{Number of people in the image}: Provides context for the individuals' emotional states, as their emotions may be influenced by those around them.
\item \textbf{Activity and Interactions}: Understanding the actions of individuals and their interactions with others can reveal more about their emotional states and the scene's context.
\item \textbf{Facial Expressions}: Key indicators of emotions, providing insight into human's feelings.
\item \textbf{Body Language}: Conveys mood, intentions, and complementing facial expressions.
\end{itemize}

\subsection{Scenario Specific Self-Ask Thinking}
\label{sec:scenario_spe_self_ask}
We delve into specific image scenarios and pose detailed questions that are relevant to the current context. To guide the model in question generation, we present an example $e_{sce}$ alongside the user question $x_{query}$, the reconstructed question $x_{rec}$, and the general self-ask question-answer pairs $x_{gen}$. This approach enables the model to focus on specific contextual elements within the image, fostering a more precise and nuanced understanding of the situation.

The process is formalized through the function $f_{ass}$, which takes into account the example scenario $e_{sce}$, user question $x_{query}$, reconstructed question $x_{rec}$, and general self-ask question-answer pairs $x_{gen}$, given the image $x_{img}$ and its corresponding emotion label $x_{emo}$:

\begin{equation}
    x_{sce} = f_{ass}(e_{sce}, x_{query}, x_{rec}, x_{gen}|x_{img}, x_{emo})
\end{equation}


